LiDAR Inertial Odometry And Mapping Using Learned Registration-Relevant Features

SLAM is an important capability for many autonomous systems, and modern LiDAR-based methods offer promising performance. However, for long duration missions, existing works that either operate directly the full pointclouds or on extracted features face key tradeoffs in accuracy and computational efficiency (e.g., memory consumption). To address these issues, this paper presents DFLIOM with several key innovations. Unlike previous methods that rely on handcrafted heuristics and hand-tuned parameters for feature extraction, we propose a learning-based approach that select points relevant to LiDAR SLAM pointcloud registration. Furthermore, we extend our prior work DLIOM with the learned feature extractor and observe our method enables similar or even better localization performance using only about 20\% of the points in the dense point clouds. We demonstrate that DFLIOM performs well on multiple public benchmarks, achieving a 2.4\% decrease in localization error and 57.5\% decrease in memory usage compared to state-of-the-art methods (DLIOM). Although extracting features with the proposed network requires extra time, it is offset by the faster processing time downstream, thus maintaining real-time performance using 20Hz LiDAR on our hardware setup. The effectiveness of our learning-based feature extraction module is further demonstrated through comparison with several handcrafted feature extractors.

==> sections/acknowledgement.tex <==
We thank the rest of the UCLA/NU SARA team for their support and feedback. 

==> sections/experiments/stress.tex <==
Time it takes for the algorithm to break, or finishes the whole sequence, with adaptive keyframing off (i.e. a keyframe every 1.0 m or 180 deg rotation)

64 GB Test:
DLIOM:
Constantly fails at around 1454 keyframes and 23 GB RAM.
Using jaccard: 1455 keyframing, 23 GB RAM
jaccard 40kf: 1504 keyframes, 24 GB RAM
All fails in 5th bag approaching the starting point

Ours:
Completes Short sequence and 2601 keyframes

32 GB 1.0 thresh Test:
DLIOM:
map node crash at around 10 GB, but front end (Odom Node) continues to run, whole thing crashes in seq 8

Ours:
Finished, 1088 keyframes, 13 GB RAM

32 GB 0.5 thresh Test:
DLIOM:
20980.13 MB, 1181 Kfs, turn into parkland from foresty region, 636s

Ours:
Finishes, 18999 MB, 2784 Kfs

\begin{figure}[t!] 
    \centering
    \includegraphics[width=\columnwidth]{images/experiment/mem_usage_long_lim30GB.png}
    \caption{Resident Set Size (MB) over time when simulating long mission by running Newer College Dataset \cite{ramezani2020newer} Short but forcing more keyframes. Here we use a machine with 32 GB of RAM to reach the limit faster. DLIOM (orange) fails after 636s and 1181 keyframes, whereas ours (green) finishes the whole trajectory with 2784 keyframes.}
    \label{fig:mem_usage}
\end{figure}
